Listening Between the Lines: Synthetic Speech Detection Disregarding Verbal Content

Recent advancements in synthetic speech generation have led to the creation of forged audio data that are almost indistinguishable from real speech. This phenomenon poses a new challenge for the multimedia forensics community, as the misuse of synthetic media can potentially cause adverse consequences. Several methods have been proposed in the literature to mitigate potential risks and detect synthetic speech, mainly focusing on the analysis of the speech itself. However, recent studies have revealed that the most crucial frequency bands for detection lie in the highest ranges (above 6000 Hz), which do not include any speech content. In this work, we extensively explore this aspect and investigate whether synthetic speech detection can be performed by focusing only on the background component of the signal while disregarding its verbal content. Our findings indicate that the speech component is not the predominant factor in performing synthetic speech detection. These insights provide valuable guidance for the development of new synthetic speech detectors and their interpretability, together with some considerations on the existing work in the audio forensics field.

==> 5_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

Vale la pena mettere una sezione come questa dove si discutono i risvolti dei risultati?

\begin{itemize}
    \item  Riflessioni sulla bontà di ASVspoof come dataset (poca generalizzazione)
    \item  Riflessioni sui dati degli altri dataset che vanno meglio su noise e basta
    \item  I detector vanno meglio sul noise -> Colpa dei detector o dei dati?
    \item  Detector che analizzano lo solo speech o solo noise -> funzionano in real world scenario?
    \item  Le condizioni in cui la ricerca svolge esperimenti sembrano lontane da casi reali
\end{itemize}


